Eventual hyperbolic dimension of entire functions and Poincar\'e functions of polynomials

Let $ P \colon \mathbb{C} \to \mathbb{C} $ be an entire function. A Poincar\'e function $ L \colon \mathbb{C} \to \mathbb{C} $ of $ P $ is the entire extension of a linearising coordinate near a repelling fixed point of $ P $. We propose such Poincar\'e functions as a rich and natural class of dynamical systems from the point of view of measurable dynamics, showing that the measurable dynamics of $ P $ influences that of $ L $. More precisely, the hyperbolic dimension of $ P $ is a lower bound for the hyperbolic dimension of $ L $. Our results allow us to describe a large collection of hyperbolic entire functions having full hyperbolic dimension, and hence no natural invariant measures. (The existence of such examples was only recently established, using very different and much less direct methods.) We also give a negative answer to a natural question concerning the behaviour of eventual dimensions under quasiconformal equivalence.

==> conformal-measure-removing.tex <==





HERE...

\begin{cor} \label{cor:ehypdim is strictly smaller for L}
Let $ P : \complexnumbers \rightarrow \complexnumbers $
 be a polynomial of degree at least $ 2 $ which is topologically Collet-Eckmann
 and whose Julia set is connected.
Let $\poincarefunction$
 be a Poincar{\'e} function associated to a repelling fixed point of $ P $.
Then,
\begin{equation*}
 \evhypdim \poincarefunction < \hypdim \poincarefunction.
\end{equation*}
\end{cor}


\wip{TODO: check this whole proof a last time}
\begin{proof}
 Let's first introduce many notations.
 Fix $r_0>0$ small so that the restriction of $ \poincarefunction $
 to the disk $ \Disk (0, |\multiplier|^2 r_0)$ is univalent.
 Let for all $ i \in \integers_{ \geq 0 } $,
 \begin{equation}
  A_i \defeq \setof{ z \in \complexnumbers : \abs{ \multiplier }^i r_0 \leq \abs{ z } < \abs{ \multiplier }^{ i + 1 } r_0 }
 \end{equation}
and
\begin{equation}
 A_P \defeq L (A_0).
\end{equation}

Let $ \basin (\infty) $ be the basin of $ \infty $  of $ P $.
Since the Julia set of $ P $ is connected
 there exists a conformal isomorphism
 $ \psi $
 from the basin of $ \infty $ of $ P $ onto the complement of the closed unit disk which conjugates $ f $ to $ z \mapsto z^d $.
 Since $ 0 $ is a repelling fixed point of $ P $  there exists an external ray $ \gamma $
 landing at $ 0 $,
 say of angle $ \theta_0 $.
 Let $ 1 < r_- < r_+  $ be such that
 $ \gamma \intersection A_P = \psi^{ -1 } \p{ \setof{ r e^{ i \theta_0 } : r_- \leq r < r_+ } } $.
 
Let $ \theta_- < \theta_0 < \theta_+ $ be such that
 the intersections of 
 $ \psi^{ -1 } \p{ \setof{ r e^{ i \theta } : r >  1, \theta_- < \theta < \theta_+ } }  $
 with the inner and outer boundary of the annulus $ A_P $
 both contain a set of the form
 $ \psi^{ -1 } \p{ \setof{ r (\theta) e^{ i \theta } : \theta_- < \theta < \theta_+ } } $
 with $ r (\theta) $ being  some function dependant on which boundary we consider.
 

Let 
$ \theta_- < \theta_{-0} < \theta_{-+} < \theta < \theta_{++} < \theta_{+0} < \theta_+ $.
Define the following sets:
 \begin{align}
  U_- & \defeq A_P \intersection \psi^{ -1 } \p{ \setof{ r e^{ i \theta } : r >  1, \theta_- < \theta < \theta_+ } }  \\
  U_0 & \defeq A_P \intersection \psi^{ -1 } \p{ \setof{ r e^{ i \theta } : r >  1, \theta_{-0} < \theta < \theta_{+0} } }  \\
  U_+ & \defeq A_P \intersection \psi^{ -1 } \p{ \setof{ r e^{ i \theta } : r >  1, \theta_{-+} < \theta < \theta_{++} } }.
 \end{align}
Then by construction $ U_-, U_0 $ and $ U_+ $ are connected simply connected subsets of $ A_P \intersection \basin (\infty) $
connecting both boundaries of $ A_P $.
 


Define for $ i \in \integers_{ \geq 0 } $
\begin{align}
 B^+_i   &   \defeq   \setof{ z = \rho^i \zeta :
                                 \zeta \in A_0,
                                 r_0 < \abs{ \zeta }
                                 \mbox{ and } L (\zeta) \notin U_+ }, \\
  B_i    &   \defeq   \setof{ z = \rho^i \zeta :
                                 \zeta \in A_0,
                                 (1 + \eps) r_0 < \abs{ \zeta } < (1 - \eps) r_0 \abs{ \multiplier }
                                 \mbox{ and }
                                 L (\zeta) \notin U_0 }, \\
  B^-_i  &   \defeq  \setof{ z = \rho^i \zeta :
                                 \zeta \in A_0,
                                 (1 + 2 \eps) r_0 < \abs{ \zeta } < (1 - 2 \eps) r_0 \abs{ \multiplier }
                                 \mbox{ and }
                                 L (\zeta) \notin U_- }.
\end{align}
We assume that $ \eps > 0 $ is small enough so that $ B^-_0 \neq \emptyset $.
Note that by construction $ B^-_i $, $ B^+_i $ and $ B_i $ are simply connected open subsets of $ \complexnumbers $.
We assume that $ B_i $ is connected (otherwise take the biggest connected component).

Now let $ n \in \integers_{ \geq 1 } $ be large enough so that
for all $ i \geq n $, $ B_i $ does not intersects the singular set of $ L $.
We consider the family $ \mathcal{Q} = \mathcal{Q} (n) $ of simply connected open sets $ Q \subset \complexnumbers $
 such that there exists $ i $ and $ j $ in $ \setof{ n, n + 1, \dots, 2 n } $
 such that 
 $ Q \subset B_j $,
 $ Q \intersection B^-_j \neq \emptyset $
 and the mapping $ L : Q \to B_i $ is a conformal isomorphism.
 For each $ Q \in  \mathcal{Q} $ we define
 \begin{equation}
  \ph_Q \defeq L_{ \restricted Q }^{ - 1 }.
 \end{equation}

 
 We will show that if $ n $ is large enough,
 the system of mappings $ \family{ \ph_Q }_{ Q \in \mathcal{Q} } $
 generates a conformal graph directed Markov system (CGDMS) and that
 the dimension of the limit set of this CGDMS is greater than
 \begin{equation}
  h \defeq \hypdim \poincarefunction.  
 \end{equation}
 For background on CGDMS compare \cite{MauldinUrbanski2003}. % should be the book ``Graph Directed Markov Systems''
 Moreover the limit set of the GCDMS will be an hyperbolic set for $ L $.



 Firstly assume that $ Q $ is an open connected set such that
 there exists $ Q_+ $ and
 some $ i, j \geq n $,
 such that
 $ L : Q_+ \to B_i^+ $  is a conformal isomorphism,
 $ Q \subset Q_+ $,
 $ L (Q) = B_i $
 and $ Q \intersection B_j \neq \emptyset $.
 We will show that by choosing $ n $ large enough,
 the mapping $ L $ is expanding
  with constants independent of $ Q, i, j $.
  Define as above $ \ph_{ Q } \defeq \p{ L_{ \restricted Q } }^{ -1 } $.
Note that there is a uniform bound on the distortions of the maps $ \ph_Q $, 
 measured in terms of the cylinder metric,
 independent of $ Q, i, j $.


  
 

Our first step is to estimate the norm of the derivative of the maps $ \ph_Q $ with respect to the cylinder metric.
We fix $ R > 1 $ and let $ F $ be the image of a ring $ \setof{ R < \abs{ z } \leq R^2 } $
 by the inverse of the B{\"o}ttcher coordinates at $ \infty $ for $ P $.
 Then there exists $ C_{\mbox{mono}} > 1 $ such that 
 for all $ \xi $ in the unbounded component of the complement of $ F $ and for all $ k \in \integers_{ \geq 0 } $
 \begin{equation} \label{eq: the derivative of the polynomial is comparable to the derivative of the high order monomial}
  C_{\mbox{mono}}^{ - 1 }
  \leq 
  \abs{ \frac{ \p{ P^k }' (\xi) }{ d^k P^k (\xi) / \xi } }
  \leq
  C_{\mbox{mono}}.
 \end{equation}
Note that by construction if $ w $ and $ \nu $ are such that $ P^{ - \nu } (w) \intersection F \neq \emptyset $
then $ P^{ - \nu } (w) \subset F $.
For all $ w $ in the unbounded component of the complement of $ F $,
let $ \nu_F = \nu_F (w) $ be the unique positive integer such that $ P^{ - \nu_F } (w) \subset F $.
Then there exists $ C_{ F } \in \realnumbers $
 independent of $ w $
 such that
\begin{equation}
 \frac{ \log \log \abs{ w } - C_{ F } }{ \log d } \leq \nu_F \leq \frac{ \log \log \abs{ w } + C_{ F } }{ \log d }.
\end{equation}
 We also assume $ n $ is large so that $ F $ is in the bounded component of the $ A_n $.
 
 Let $ i, j \in \setof{ n, \dots, 2 n } $ and let
 $ z \in B_j $ be such that $ L (z) \in B_i $.
 Then from Observation \ref{obs:preimage structure}
 it follows that
 $ L' (z) = \frac{ 1 }{ \rho^j } \p{ P^j }' (\zeta) L' (z / \rho^j) $
 where $ \zeta \in A_P $ is 
 \wip{ $ \zeta = L \p{ z / \rho^j } $. }
 Let $ w = L (z) $, $ \nu = \nu_F (w) $ and $ \xi = P^{ j - \nu } (\zeta) $.
 Then
 \begin{equation}
  \cylnorm{ \Deriv L (z) } = \abs{ L' (z / \rho^j) \frac{ z }{ \rho^j } \frac{ \p{ P^{ \nu } }' (\xi) }{ w } \p{ P^{ j - \nu } }' (\zeta) }. 
 \end{equation}
The factor $ \abs{ L' (z / \rho^j) \frac{ z }{ \rho^j } } $ is comparable to a constant independently from $ i, j, z, n $.
By \eqref{eq: the derivative of the polynomial is comparable to the derivative of the high order monomial}
 the term $ \abs{ \frac{ \p{ P^{ \nu } }' (\xi) }{ w } } $
 is comparable to $ d^{ \nu } \approx \log \abs{ w } $ independently from $ i, j, z, n $.
 Hence there exists $ C_{ deriv } > 1 $ independent from $ i, j, n, z, \zeta $ such that
 \begin{equation}
  C_{ deriv }^{ -1 } %\log \abs{ w } \abs{ \p{ P^{ j - \nu } }' (\zeta) }
  \leq
  \frac{ \cylnorm{ \Deriv L (z) } }{ \abs{ \p{ P^{ j - \nu } }' (\zeta) }  \log \abs{ w } }
  \leq
  C_{ deriv } .
 \end{equation}
  Moreover it follows from Lemma \ref{lem: derivative of polynomial bounded from below on the basin of infinity}
  that $ \abs{ \p{ P^{ j - \nu } (\zeta) }' } $ is bounded from below away from $ 0 $
  independently from $ i, j, \zeta, z, n $.
 
 
 Hence if $ n $ is large enough there exists $ k_{ \mathcal{Q} } > 1 $
 such that for all $ Q \in \mathcal{ Q } $ and all $ z $ in the domain of $ \ph_Q $,
 $ \cylnorm{ \Deriv \ph_Q (z) } \leq k_{ \mathcal{Q} }^{ - 1 } $.
 Moreover $ k_{ \mathcal{Q} } \tendsto \infty $ as $ n \tendsto \infty $.
 

Remark that the diameter of $ B_i $ is uniformly bounded independently from $ i $ with respect to the cylindrical metric.
 It follows that for any $ \eta > 0 $ one can find $ n $ such that
 the cylindrical diameter of $ \ph_Q (B_i) $ is smaller than $ \eta $.
 
We use this to show that the system is not empty for $ n $ large enough.
 Choose for any $ i \geq $ a point $ c_i \in B_{i}^- $.
 Then from Observation \ref{obs:preimage structure} and Proposition \ref{prop:???}
 it follows that $ L^{ -1 } (c_i) \intersection B_j $ 
 is not empty for any $ j \geq n $
 and $ n $ large enough (independently of $ i $).
 
By the previous considerations this means that on can find $ Q $ as above such that
$ \ph_Q (B_i) \subset B_j $. 
This shows that not only the system is not empty but also that it is $ 2 $-irreducible.
Hence we have an irreducible CGDMS.
We can estimate the dimension of its limit set by using thermodynamical formalism.

Indeed 
let's compute the $p$th partition function with respect to the cylinder metric:
\begin{align*}
 & 
  \familysum{i_1=n}{\widthconst n}
  \cdots
  \familysum{i_{p+1}=n}{\widthconst n}
  \familysum{\alpha_1=1}{\alpha_{i_1,i_2}}
   \cdots
  \familysum{\alpha_p=1}{\alpha_{i_p,i_{p+1}}}
   \left\| \left(\ph_{i_1,i_2,\alpha_1}
                 \composedwith \cdots \composedwith
                 \ph_{i_p,i_{p+1},\alpha_p}\right)' \right\|_{\cyl}^t \\
  & \geq
  \kappa_1
  \familysum{i_1=n}{\widthconst n}
  \cdots
  \familysum{i_{p+1}=n}{\widthconst n}
  \familysum{\zeta_1\in A_0\intersection P^{-i_1}(A_{i_2})}{}
  \cdots
  \familysum{\zeta_p\in A_0\intersection P^{-i_p}(A_{i_p+1})}{}
   (i_1\cdot\dots\cdot i_p)^{-t}
   \left|P^{i_1-\nu_{i_2}}(\zeta_1)\right|^{-t}
   \cdot \dots \cdot
   \left|P^{i_p-\nu_{i_{p+1}}}(\zeta_p)\right|^{-t} \\
  & \geq
  \kappa_2
  \familysum{i_1=n}{\widthconst n}
  \cdots
  \familysum{i_{p+1}=n}{\widthconst n}
   n^{-p t}
   \partitionfunction(P^{i_1-\nu_{i_2}}_{\restricted N},t)
   \cdot \dots \cdot
   \partitionfunction(P^{i_p-\nu_{i_{p+1}}}_{\restricted N},t) \\
  & \geq
   \kappa_3 n^{p(1-t)+1}.
\end{align*}
(where $\kappa_i>0$ are constants independent of $n,p$).

 

 



\end{proof}



HERE...
\begin{proof}[Old not working proof - work in progress]

\renewcommand{\widthconst}{{C_0}}

$\widthconst > 2$

Fix $r_0>0$ small so that the restriction of $\poincarefunction$
 to a neighborhood of the disk $D_0 = \Disk (0, |\multiplier| r_0)$ is univalent.
 Let $A_0 = D_0 \setcomplement \Disk (0, r_0)$,

 Let $\eps>0$ such that $\eps<|\multiplier|-1$.
 Define, for $i>0$
 \begin{equation*}
 A_i=\left\{z:
 (1+\eps)|\multiplier|^i r_0 \leq z \leq (1-\eps)|\multiplier|^{i+1} r_0
 \mbox{ and }
 \realpart (z)\geq 0\mbox{ or }|\imaginarypart(z)|\geq\eps\right\}.
 \end{equation*}

Consider, for $n\in\nonzeronaturalnumbers$, the family of simply connected domains
 $(A_i)_{i=n,\dots,\widthconst n}$.
Assume $n$ large enough so that $A_i$ doesn't contain any singular value of $L$
 for any $i\geq n$.

Consider the conformal graph directed Markov system
 consisting of the inverse branches of $L$ on $A_i$,
 for $i=n,\dots,\widthconst n$,
 and whose image is contained in $\familyunion{i=n}{\widthconst n}A_i$.
 
No take preimages by the second iterate
say
choose a FIXED big disk (is it really necessary?)
iterates must stay inside the complement of this disk
can also restrict to iterates in the union of the distant annulus
 and the bounded region in the complement of this annulus
 (probably sufficient, if it helps?).

TTTTT
$\ph_{i,j,\alpha}:A_i\rightarrow X_{i,j,\alpha}$
 where $X_{i,j,\alpha}\subset A_j$ is a simply connected domain
 on which $\poincarefunction$ is injective
 and $\ph_{i,j,\alpha}=\poincarefunction_{\restricted X_{i,j,\alpha}}^{-1}$.
 The index $\alpha$ ranges over all such domains.
 
claim: this is a nonempty system, and most of the branches are here.

It is $2$-irreducible.

Admissible compositions $\ph_{i,j,\alpha}\composedwith\ph_{i',j',\alpha'}$
 such that $j=i'$.

Let's compute the $p$th partition function with respect to the cylinder metric:
\begin{align*}
 & =
  \familysum{i_1=n}{\widthconst n}
  \cdots
  \familysum{i_{p+1}=n}{\widthconst n}
  \familysum{\alpha_1=1}{\alpha_{i_1,i_2}}
   \cdots
  \familysum{\alpha_p=1}{\alpha_{i_p,i_{p+1}}}
   \left\| \left(\ph_{i_1,i_2,\alpha_1}
                 \composedwith \cdots \composedwith
                 \ph_{i_p,i_{p+1},\alpha_p}\right)' \right\|_{\cyl}^t \\
  & \geq
  \kappa_1
  \familysum{i_1=n}{\widthconst n}
  \cdots
  \familysum{i_{p+1}=n}{\widthconst n}
  \familysum{\zeta_1\in A_0\intersection P^{-i_1}(A_{i_2})}{}
  \cdots
  \familysum{\zeta_p\in A_0\intersection P^{-i_p}(A_{i_p+1})}{}
   (i_1\cdot\dots\cdot i_p)^{-t}
   \left|P^{i_1-\nu_{i_2}}(\zeta_1)\right|^{-t}
   \cdot \dots \cdot
   \left|P^{i_p-\nu_{i_{p+1}}}(\zeta_p)\right|^{-t} \\
  & \geq
  \kappa_2
  \familysum{i_1=n}{\widthconst n}
  \cdots
  \familysum{i_{p+1}=n}{\widthconst n}
   n^{-p t}
   \partitionfunction(P^{i_1-\nu_{i_2}}_{\restricted N},t)
   \cdot \dots \cdot
   \partitionfunction(P^{i_p-\nu_{i_{p+1}}}_{\restricted N},t) \\
  & \geq
   \kappa_3 n^{p(1-t)+1}.
\end{align*}
(where $\kappa_i>0$ are constants independent of $n,p$?).

The set $N$ is a large neighborhood of the Julia set of $P$

By the choice of $t$,
 the partitions functions of $P$ are uniformly bounded away from $0$ on $N$
 by a positive constant $\kappa_0$.






\end{proof}



\begin{proof}
 \wip{NOTE: can probably be replaced by a CGDMS}

Fix $r_0>0$ small so that the restriction of $\poincarefunction$
 to a neighborhood of the disk $D_0 = \Disk (0, |\multiplier| r_0)$ is univalent.
 Let $A_0 = D_0 \setcomplement \Disk (0, r_0)$,

Define, for $n>0$
\begin{equation*}
 Q = Q_n \defeq
 \setof{ z \in \juliaset (\poincarefunction) : |\multiplier|^n r_0 \leq |z| \leq |\multiplier|^{2 n} r_0 }.
\end{equation*}
Assume $n$ large enough so that
$\abs{\multiplier}^n r_0 > 1$ and
$Q$ is nonempty and doesn't contain any singular value of $L$.

Consider the set $X$ of points in $Q$ whose orbits never escape $Q$:
\begin{equation*}
 X \defeq \left\{z \in Q: \forall i\in\naturalnumbers, \poincarefunction^{i}(z)\in Q\right\}.
\end{equation*}

Let $t \defeq \evhypdim \poincarefunction $.
Our aim is to show that $\hausdorffdimension X > t$.
We compute the first partition of $\poincarefunction$ on $X$ with respect to the cylinder metric.
Let $w\in Q$, then,
\adz{\begin{equation*}
 Z(w) \defeq \cylpartfun \p{t, \poincarefunction_{\restricted Q}, w} 
  = \familysum{z \in \poincarefunction^{-1}(w)\intersection Q}{}
   \frac{\left|w\right|^t}{|z|^t\left|\poincarefunction'(z)\right|^t}.
\end{equation*}}

Then, from Lemma \ref{lem:lower bound on part of 1st pratition function of L}
 it follows that there exists $C > 0$ (independent of $w$ and $n$) such that
\begin{equation*}
 Z (w) \geq
   C \familysum{k = n}{2 n - 1}
    n^{1 - t}
    = 
   C n^{2 - t}.
\end{equation*}

\begin{claim}
There exists $\kappa > 1$
 such that for all $n$ large enough and for all
 $z, z' \in Q \intersection \poincarefunction^{-1}(Q)$,
 \adz{$\frac{\cylnorm{\Deriv \poincarefunction(z)}}
       {\cylnorm{\Deriv \poincarefunction(z')}}
   \leq \kappa$}.
\end{claim}
\begin{proof}[Proof of the claim]
\newcommand{\poinfunclogtransf}{\tilde{\poincarefunction}}
 Let $\poinfunclogtransf$ be the logarithmic transform of $\poincarefunction$.
 Then \adz{$ Q = \exp \left(\tilde{Q}\right) \intersection \juliaset (L) $ }
 where
\begin{equation*}
  \tilde{Q} = n S_0 + \log r_0 + \frac{3}{2} n \log |\multiplier|,
\end{equation*}
and $n S_0$ is the homothetic image of factor $n$ of the set
\begin{equation*}
 S_0 = \left\{ z:
           \left|\imaginarypart (z)\right| < \pi,
           \left|\realpart (z)\right| < \frac{1}{2} \log |\multiplier|
       \right\}.
\end{equation*}
Inverse branches $G$ of $\poinfunclogtransf$
 are defined on the the set $\frac{3}{2} n S_0 + \log r_0 + \frac{3}{2} n \log |\multiplier|$
 for all $n$ large enough.
 Hence by Koebe distortion theorem, there exists $\kappa > 1$
 such that for all
 $\tilde{z},\tilde{z}' \in \tilde{Q} \intersection \poinfunclogtransf^{-1}\left(\tilde{Q}\right)$,
 $\frac{\left|\poinfunclogtransf'\left(\tilde{z}\right)\right|}
       {\left|\poinfunclogtransf'\left(\tilde{z}'\right)\right|}
     \leq \kappa$.
Then, the claim follows from the identity
 \adz{$\left|\poinfunclogtransf'\left(\tilde{z}\right)\right|
   = \cylnorm{ \Deriv \poincarefunction \left(e^{\tilde{z}}\right)}$.}
\end{proof} 


Since $t<2$,
we can choose $n$ large enough so that the first partition function is bigger than $\kappa^t$.
This implies that the sequence of partition functions
 of the iterates of $\poincarefunction$ on $Q$ explodes exponentially fast.
As a consequence the pressure on $X$ is positive,
 hence the Hausdorff dimension of $X$ is greater than $t$
 (see e.g. \cite{PrzytyckiUrbanski2010}, Chapter 9).
\end{proof}














































HERE2

\begin{cor} \label{cor: smooth ergodic theory for poincare functions}
 Let $P$ be a polynomial of degree at least $2$
  with connected Julia set and which is topologically Collet-Eckmann.
Let $\poincarefunction$
 be a Poincar{\'e} function associated to a repelling fixed point of $P$.
 Assume that $\poincarefunction$ is hyperbolic.
 
Then $\poincarefunction$
 admits a $h$-conformal measure $m$ supported on its radial Julia set
 and whose exponent $h$ is equal to the hyperbolic dimension of $\poincarefunction$.
 The measure $m$ is ergodic conservative
 and there exists a unique $f$-invariant probability Borel measure which is equivalent to $m$.
\end{cor}

\begin{proof}
This is a direct consequence of
 item \ref{it:theta is hypdim of P} of Corollary \ref{cor:theta is hypdim of P},
 Corollary \ref{cor:ehypdim is strictly smaller for L}
 and Theorem \ref{thm: general theorem on existence of conformal and invariant equivalent measures}.
\end{proof}






\begin{proof}[Proof of Theorem \ref{thm:nicelinearisers}]
\adz{
 Since the Julia set of $ P $ is connected $ \hypdim P \geq 1 $.
 From Lemma \ref{lem: evhypdim L leq hypdim P for TCE J connected P}
 and Theorem \ref{thm:evhypdim ge hypdim}
 it follows that $ \hypdim P = \evhypdim L $.
 Corollary \ref{cor:ehypdim is strictly smaller for L} shows that $ \hypdim L > \evhypdim L $.
}

\adz{
 The existence of the conformal and ergodic equivalent measures follows from
 Corollary \ref{cor: smooth ergodic theory for poincare functions}.
}

 \adz{
 The inequality $ \hypdim L < 2 $ then follows from the existence of a conformal measure for $ L $.
 }
 
 \adz{
Finally since $P$ is a polynomial,
the order of growth of the lineariser $\poincarefunction$ is finite (see \cite{EremenkoSodin1990}).
For functions of finite order in class $\classb$, the dimension
  of the Julia set is $2$ (Theorem A of \cite{Baranski2008}).}
\end{proof}


==> conformal-measure.tex <==






















\section{Conformal and invariant measures for Poincar{\'e} functions} \label{sec:conformal measures for linearizers}

The aim of this section is to study the behavior of the partition function and vanishing exponent of 
 the Poincar{\'e} function of a polynomial, in particular Corollary \ref{cor:theta is hypdim of P}.
 
 

 
We will need the following lemma extracted from \cite{Przytycki1999}, Lemma 3.1 and proof of Theorem 3.3.

\begin{lem} \label{lem: distortion between two points}
 Let $ f $ be a 
 polynomial
 map of degree $ \geq 2 $.
 Then there exists
 $ \kappa \geq 1 $,
 and
 $ E \subset \complexnumbers $ a subset of the closure of the critical orbits of $ f $
 such that 
 $ \hausdorffdimension (E) = 0 $
 and for all
 $ z_0, z_1 \in \riemannsphere \setcomplement E $
 and all $ n \in \positiveintegers $
 \begin{equation}
  \frac{ \abs{ \p{ f^n }' (z_1) } }{ \abs{ \p{ f^n }' (z_0) } } \leq \kappa^{ n^{ 3/4 } }.
 \end{equation}
\end{lem}


\begin{rem} \label{rem: exceptional set can be forward invariant}
 By replacing $ E $ by $ \familyunion{ n \in \integers_{ \geq 0 } }{} f^n (E) $
 we can assume that $ E $ is forward invariant while still having Hausdorff dimension $ 0 $.
\end{rem}

























\begin{lem} \label{lem:positive lower bound on P poincare sums}
Let $P$ be a topologically Collet-Eckmann polynomial of degree at least $2$.
Let $U$ be a bounded neighborhood of the Julia set $\juliaset(P)$ of $P$
 such that $P^{-1}(U)\subset U$
 and let $A_P$ be a bounded open set intersecting $\juliaset(P)$.
 
Then for all $t \leq \hypdim (P)$, 
 there exits $\delta > 0$
 such that for all $\xi \in U$,
 and all $ j \in \integers_{ \geq 0 } $,
\begin{equation} \label{eq:positive lower bound on P poincare sums}
 \familysum{\zeta \in P^{-j}(\xi) \intersection A_P }{}
  \abs{ \left(\PoincareFunctionPolynomial^{j}\right)'(\zeta) }^{-t}
 \geq \delta.
\end{equation}

Moreover
if $ t < \hypdim (P) $ the inequality \eqref{eq:positive lower bound on P poincare sums}
 holds even if $P$ is not topologically Collet-Eckmann.
\end{lem}

\begin{proof}
Let $ \xi \in U $ and $ j \in \naturalnumbers $.
 Let $ s = s \p{ U, A_P } \in \naturalnumbers $ be such that
 \begin{equation*}
  P^{ s } \p{ A_P } \supset U.
 \end{equation*}
We assume $ j > s $. Then, by definition of $ s $,
 for every $ \zeta' \in P^{ - (j - s) } (\xi) $,
 there exist $ \zeta \in A_P $ such that $\zeta' = P^s (\zeta)$.
 This implies that $ \zeta \in P^{-j} (\xi) \intersection A_P $.
 
Consequently,
\begin{equation}
 \familysum{\zeta \in  P^{-j}(\xi) \intersection A_P }{}
    \abs{\p{\PoincareFunctionPolynomial^{j}}'(\zeta)}^{-t}
 \geq
   \p{\sup_{U} \abs{{P^s}'}}^{ - t }
   \familysum{\zeta' \in  P^{-(j - s)}(\xi)}{}
     \abs{\p{\PoincareFunctionPolynomial^{j - s}}'(\zeta')}^{-t}.
\end{equation}\adz{
Hence it is sufficient to show that the inequality \eqref{eq:positive lower bound on P poincare sums} holds
 in the case where $ A_P $ contains the whole Julia set.

Fist assume that $ t < \hypdim (P) $.
We use the notation
\begin{equation}
 Z_n (t, z) \defeq \familysum{ \zeta \in P^{ -n } (z) }{} \abs{ {P^n}' (\zeta) }^{ -t }.
\end{equation}
From Lemma \ref{lem: distortion between two points}
and Remark \ref{rem: exceptional set can be forward invariant}
it follows that
there exists $ \kappa > 1 $,
independent from $ t, n, z_0 $ and $ z_1 $,
such that
 \begin{equation} \label{eq:bound on the partition function distortion for the polynomial}
  Z_n (t, z_0) / Z_n (t, z_1) \leq \kappa^{ t n^{3/4} }
 \end{equation}
 for any $ n \geq 1 $ and
 and
for any $ z_0, z_1 \in A_P $ outside a forward invariant set $ E $ of Hausdorff dimension $ 0 $.
 In particular since the value of the pressure for $ P $ at exponent $ t $ is positive there exists an increasing sequence of positive integers
 $ n_j $ 
 such that for all $ z \in A_P \setcomplement E $
 \begin{equation}
  \lim_{ j \tendsto \infty } \frac{ 1 }{ n_j } \log Z_{ n_j } (t, z) \eqdef \pressure (t) > 0.
 \end{equation}
 Fix $ z_* \in  \juliaset (P) \setcomplement E $ and let $ \beta_j > 1 $, $ \beta_j \tendsto e^{ \pressure (t) } $ 
 be such that $ Z_{ n_j } (t, z_*) \geq \beta_j^{ n_j } $.
 
 Let $ z \in A_P \setcomplement E $ and  $ p \in \positiveintegers $ then by the above and inequality \eqref{eq:bound on the partition function distortion for the polynomial}
 \begin{equation}
  Z_{ p n_j } (t, z) \geq \beta_j^{ p n_j } \kappa^{ - t p n_j^{ 3/4 } }.
 \end{equation}
 This implies that if $ j $ is chosen so that $ n_j $ is large enough the sequence of partition functions $ Z_{ p n_j } (t, z) $
 converge to $ \infty $ exponentially in $ p \tendsto \infty $ (with a lower bound on the rate which is independent of $ z $).

 The derivative of $ P $ is bounded by some constant $ M > 0 $ on $ A_P $
 hence by the above one can find $ C_1  > 0 $
 and $ \beta > 1 $
 both independent of $ n $ and $ z $
 such that for any $ z \in \juliaset (P) \setcomplement E $
 \begin{equation}
  Z_n (t, z) \geq C_1 \beta^n.
 \end{equation}
 
 Note that the function
 $ \xi \mapsto \familysum{\zeta \in P^{-j}(\xi) \intersection A_P }{} \abs{ \left(\PoincareFunctionPolynomial^{j}\right)'(\zeta) }^{-t} $
 is upper semicontinuous outside the postcritical set of $ P $ and infinite on the postcritical set.
 Since the exceptional set $ E $ has zero two dimensional Lebesgue measure
 it follows that the lower bound \eqref{eq:positive lower bound on P poincare sums}
 is valid for all $ \xi \in U $.

 Since $ U $ is bounded it follows that we can also find a positive lower bound $ \delta > 0 $
 for any $ j \in \integers_{ \geq 0 } $.
}
  

The case where  $ t = \hypdim (P) $ and $ P $ is topologically Collet-Eckmann
follows directly from the following result for thermodynamic formalism
(see for example \cite[Theorem B]{PrzytyckiRiveraLetelier2007}).
\begin{lem}
 Let $ P $  be a topologically Collet-Eckmann polynomial map of degree at least $ 2 $.
 Let $ U $ be a neighborhood of the Julia set $ \juliaset (P) $ of $ P $
 and $ h $ be the Hausdorff dimension of $ \juliaset (P) $.
 
 Then there exists $ \delta_0 > 0 $ such that 
 for all $ w \in U $ and all $ n \in \integers_{ \geq 0 } $
 \begin{equation}
  \familysum{ z \in P^{ -n } (w) }{} \abs{ \p{ P^n }' (z) }^{ -h } \geq \delta_0.
 \end{equation}
\end{lem}
\end{proof}




























\begin{lem} \label{lem:lower bound on part of 1st pratition function of L}
Assume $P$ is a polynomial of degree at least $2$ with connected Julia set.
 Assume that $P$ has a repelling fixed point of multiplier $ \rho $
 and let $\poincarefunction$ be a Poincar{\'e} function for this fixed point.
 Let $r_0 > 0$ be such that the map
  $\poincarefunction$ is univalent on a neighborhood of
  $\closure{\disk(0, r_0 |\multiplier|)}$.
\adz{  For $ n \geq 0 $ define
  \begin{equation}
   A_n \defeq \setof{ z : r_0 |\multiplier|^n < |z| \leq r_0 |\multiplier|^{n+1} }.
  \end{equation}}


\begin{enumerate}
\item \label{it:bound of partit fun of L, below hypdim}
If $ t < \hypdim (P) $, then there exists
 $ \delta_- > 0 $ and
 $ k_0 \geq 1 $ such that,
 for all $ k, \ell \geq k_0 $
 and for all $w \in A_{\ell}$,
\begin{equation}\label{eq:lower bound on one part of the partition function of L}
 \familysum{z \in \poincarefunction^{-1}(w) \intersection A_k}{}
  \adz{\mcylnorm{\Deriv L(z)}^{-t}}
    \geq 
  \delta_- \ell^{1 - t} \adz{.}
\end{equation}

\item \label{it:bound of partit fun of L, above hypdim}
If $t > \hypdim (P)$, then there exists $\kappa > 0$, $\beta > 0$, $ \delta_+ > 0 $
 and a natural number $k_0$
 such that for all $k, \ell \geq k_0$
 and all $w \in A_\ell$
 satisfying $L^{-1}(w) \intersection A_k \neq \emptyset $,
\begin{equation}\label{eq:upper bound on one part of the partition function of L}
 \familysum{z \in \poincarefunction^{-1}(w) \intersection A_k}{}
  \mcylnorm{ \Deriv L (z) }^{-t}
    \leq 
  \delta_+ \ell^{1 - t} e^{- \beta (k - \nu)},
\end{equation}
 where $\nu = \nu (w)$ depends on $w$ and is a $\bigo (\log |w|)$
 with constants independent of $ \ell, k \geq k_0 $.

\item
If $t = \hypdim (P)$
 and if the polynomial $P$ is topologically Collet-Eckmann
 then the conclusion of \adz{point} \ref{it:bound of partit fun of L, below hypdim}
 still holds.
\end{enumerate}

 
\end{lem}





\begin{proof}
If $ k_0 $ is large enough
and $ \ell \geq k_0 $ 
and $ k \geq k_0 $
then for all $ w \in A_{ \ell } $
and all $ z \in L^{ -1 } (w) \intersection A_k $,
 $\cylnorm{ \Deriv \poincarefunction (z) } = \mcylnorm{ \Deriv \poincarefunction (z) } $.
 We will assume that this is the case
 and proceed to prove the inequalities in the statement directly with the cylindrical norm.

 
Let $d \geq 2$ be the degree of $P$ and let $\eps > 0$ be arbitrary.
Then there exists a neighborhood $\nonmonomialneighborhood$
 of the Julia set of $\PoincareFunctionPolynomial$
satisfying the following properties.
Denote by $\filledjuliaset(\PoincareFunctionPolynomial)$
 the filled Julia set of $\PoincareFunctionPolynomial$
 and let
 $ \psi : \complexnumbers\setcomplement\filledjuliaset (P) \rightarrow \complexnumbers\setcomplement \closure{ \unitdisk } $
 be the B{\"o}ttcher coordinates 
 of $ P $ near infinity.
Then there is $\nonmonomialneighborhoodradius>1$ such that
 $ \nonmonomialneighborhood = \psi^{-1} \p{ \closure{ \disk (0, \nonmonomialneighborhoodradius) } } $
 and for all $\nu \geq 1$ and all $\xi$ in the complement of $\nonmonomialneighborhood$,
\begin{equation} \label{eq:monomial comparison}
 \left|\frac{ \PoincareFunctionPolynomial^{\nu}(\xi)}{\xi^{d^\nu}} - 1 \right| \leq \eps, \\
 \left|\frac{ \left(\PoincareFunctionPolynomial^{\nu}\right)'(\xi)}
              {{d^\nu} \PoincareFunctionPolynomial^{\nu}(\xi) / \xi}
       - 1 \right| \leq \eps.
\end{equation}

We also assume that $ R_P $ is large enough so that $ N $ contains the unit disk.
Given such $ N $, there exists a constant $ C_1 > 0 $ 
 such that for all $\xi \in \complexnumbers \setcomplement \nonmonomialneighborhood$,
\begin{equation} \label{eq:number of iterations from fund ann}
 C_1^{-1} \leq \frac{\log \abs{ P^{ \nu } (\xi) } }{ d^\nu \log \abs{ \xi } } \leq C_1.
\end{equation}


Define 
\begin{equation*}
 \monomialfundamentalannulus
   \defeq \psi^{-1}\left(
                \left\{
                  z : \nonmonomialneighborhoodradius < |z| \leq \nonmonomialneighborhoodradius^d
                \right\}
               \right).
\end{equation*}

Let $R > 0$ be large enough so that the set 
 $\nonmonomialneighborhood \union \monomialfundamentalannulus$
 lies inside the disk of radius $R$ centered at the origin.
This allows to define, for $w$ outside that disk,
\begin{equation} \label{eq: definition of the set of preimages near the fixed point}
 \setofmonomialpreimages
   = \setofmonomialpreimages (w)
   \defeq \PoincareFunctionPolynomial^{-\nu}(w) \intersection \monomialfundamentalannulus,
\end{equation}
 where $\nu = \nu (w) \geq 1$ is the smallest natural number such that
\begin{equation}
 P^{ - \nu } (w) \intersection \monomialfundamentalannulus \neq \emptyset.
\end{equation}
It follows from the definition of $\monomialfundamentalannulus$
 that $ P^{ - \nu } (w) \subset F $
 and
 the cardinality of the set $\setofmonomialpreimages$
 is equal to $ d^\nu $.
Moreover, from \eqref{eq:number of iterations from fund ann},
 it follows that $d^\nu$ is comparable to $\log |w|$.
 
Recall that $r_0 > 0$ is such that the map
  $\poincarefunction$ is univalent on a neighborhood of
  $\closure{\disk(0, r_0 |\multiplier|)}$.
  Define 
\begin{equation*}
 A_P \defeq L\left(\left\{z : r_0 < |z| \leq r_0 |\multiplier| \right\}\right).
\end {equation*}
 
Assume $ \abs{ w } > R $ and let $ \mu = \mu (w) $ be the smallest natural number such that
\begin{equation}
  P^{ - \mu } (w) \intersection A_P \neq \emptyset.
\end{equation}
 Note that $ \mu $ is also comparable to $ \log |w| $.
 We also assume that $ R_P $ is large enough so that $ A_P \subset N $.

 
For a given $ k \geq 1 $ and for $ |w| > R $, let
\begin{equation}
 \partitionfunction (w) \defeq
   \familysum{z \in \poincarefunction^{-1}(w) \intersection A_k}{}
     \cylnorm{ \Deriv L(z) }^{-t}
\end{equation}
and for $ k \geq \mu (w) $ and $ \xi \in \setofmonomialpreimages $,
 define
\begin{equation} \label{eq: definition of the local partition function for P}
 \polypartifuns_\xi
    \defeq
     \familysum{\zeta \in P^{-(k-\nu)} (\xi) \intersection A_P}{}
       \abs{ \left(\PoincareFunctionPolynomial^{k - \nu}\right)'(\zeta) }^{-t}.
\end{equation}
\adz{
Then, using Observation \ref{obs:preimage structure},
\begin{equation}
 Z (w)
 =
 \sum_{ \xi \in \Xi }
 \sum_{ \zeta \in P^{ - (k - \nu) } (\xi) \intersection A_P }
 \cylnorm{ \Deriv L (z) }^{ - t }
\end{equation}
with $ L (z / \rho^k ) = \zeta $.
From
 Observation \ref{obs:preimage structure},
 $ \cylnorm{ \Deriv L (z) } $ is comparable to $ \abs{ \frac{ \p{P^{ \nu }}'(\xi) }{ w } } \abs{ \p{ P^{k - \nu} }' (\zeta) } $.
}

Then from
 and the second inequality in \eqref{eq:monomial comparison},
 it follows that there is a constant $C_2 > 1$ independent of $ k $ and $ w $ such that
\begin{equation}\label{eq: partition function equivalence}
   C_2^{-1}
   \familysum{\xi \in \setofmonomialpreimages}{}
     d^{-t \nu} \polypartifuns_\xi
 \leq
     \partitionfunction (w)
 \leq 
     C_2
     \familysum{\xi \in \setofmonomialpreimages}{}
      d^{-t \nu} \polypartifuns_\xi.
\end{equation}


If $t < \hypdim (P)$,
 or if $t = \hypdim (P)$ and $P$ is topologically Collet-Eckmann,
 then inequality \eqref{eq:lower bound on one part of the partition function of L}
 follows from Lemma \ref{lem:positive lower bound on P poincare sums}
 \adz{ and the fact that $ d^\nu > C_3 \ell $
 for $ k_0 $ large enough where $ C_3 > 0 $ is some suitable constant. }



Now suppose $t > \hypdim (P)$.
Let $ \xi_0 \in F $. 
Since the Julia set of $ P $ is connected it follows that $ F \intersection E = \emptyset $
where $ E $ is the exceptional set mentioned in Lemma \ref{lem: distortion between two points}.
It follows from \cite{Przytycki1999}
that
 there exists constants $ \beta_0 > 0 $ % and $C_4 > 0$
 such that for all $ k > \nu $
\begin{equation*}
 \polypartifuns_{ \xi_0 }
 \leq \familysum{ \zeta \in\zeta \in P^{-(k-\nu)} (\xi) }{} \abs{ \p{ P^{ k - \nu } }' (\zeta) }^{-t}
 \leq e^{ - \beta_0 (k - \nu) }.
\end{equation*}
 Using Lemma \ref{lem: distortion between two points} and the above inequalities
 we obtain that for all $ \xi \in F $ and all $ k > \nu $,
 \begin{equation}
  \polypartifuns_{ \xi } \leq e^{ \beta (k - \nu) }
 \end{equation}
 where $ \beta = \beta_0 + \log \kappa > 0 $.
 
This and the fact that $ d^\nu $ is comparable to $ \ell $ for $ k_0 $ large
 implies inequality \eqref{eq:upper bound on one part of the partition function of L}.
\end{proof}













\begin{cor} \label{cor:theta is hypdim of P}
 Let $\poincarefunction$ be a lineariser of a
 polynomial $P$ of degree $d \geq 2$ with connected Julia set. % and such that $\hypdim (P) > 1$.
 Then we have the following.
\begin{enumerate}
\item
 For any $t < \hypdim (P)$ and for all $w$ large enough,
 \begin{equation*}
   \mcylpartfun (t, \poincarefunction, w) = +\infty.
 \end{equation*}

\item \label{it:theta is hypdim of P}
\begin{equation*}
 \vanishingexponent (\poincarefunction) = \hypdim (P).
\end{equation*}

\end{enumerate}
\end{cor}

\begin{proof}
First assume $t < \hypdim (P)$
Let $w$ be large enough.
Then if follows from
 item \ref{it:bound of partit fun of L, below hypdim} of
 Lemma \ref{lem:lower bound on part of 1st pratition function of L}
 that there exists $ C > 0 $ such that
\adz{\begin{equation*}
 \mcylpartfun (t, \poincarefunction, w)
   \geq
  \familysum{n=n_0}{+\infty} C (\log |w|)^{\frac{ 1 - t}{2}} = + \infty,
\end{equation*}}
where $n_0 = n_0 (w)$ comes from Observation \ref{obs:preimage structure} and Lemma \ref{lem:lower bound on part of 1st pratition function of L}.
 
Now suppose $t > \hypdim (P)$.
 From item \ref{it:bound of partit fun of L, above hypdim} of
 Lemma \ref{lem:lower bound on part of 1st pratition function of L}
 it follows that there exists (another) $ C  > 0$ and $ \beta > 0 $ such that,
  for all $ w $ large,
\adz{\begin{equation*}
 \mcylpartfun (t, \poincarefunction, w)
  \leq
 C_1 \familysum{n = n_0}{+\infty} (\log |w|)^{2 (1 - t)} e^{- \beta (n - \nu)},
\end{equation*}}
where $\nu = \nu (w) \leq n_0$ is a $\bigo (\log |w|)$.
Hence $\mcylpartfun (t, \poincarefunction, w) \leq C_2 (\log |w|)^{1 - t}$
 for some constant $C_2 > 0$.
Since $t > 1$, this implies that
 $\mcylpartfun (t, \poincarefunction, w) \tendsto 0$
  as $|w| \tendsto \infty$.
\end{proof}







We will need the following lemma in the proof of next corollary.
\begin{lem}[See \cite{GraczykSmirnov1998}, p.86, Lemma 6] \label{lem: derivative of polynomial bounded from below on the basin of infinity}
 Let $ P : \complexnumbers \rightarrow \complexnumbers$
 be a polynomial of degree $ d \geq 2 $
 and such that its  basin at infinity $ V $ is simply connected.
 Let $ \ph : \unitdisk \to V $
 be the B{\"o}ttcher isomorphism with $ \ph (0) = \infty $.
 Let $ 0 < r < 1 $. 
 
 Then
 there exists a constant $ C > 0 $ %independent of ...
 such that for all $ w \in \ph \p{ \setof{ \xi : r^2 \leq \abs{ \xi } \leq r } } $,
 all $ n \in \nonnegativeintegers $
 and all $ z \in P^{ -n } (w) $,
 \begin{equation}
  \abs{ \p{ P^n }' (z) } \geq C.
 \end{equation}
\end{lem}

\begin{proof}
\wip{need to check this proof}

Since $ \boundary V $ is bounded it follows from Cauchy formula that
for all $ s \in \openinterval{ 0, 1 } $ there exists $ C_s > 0 $
such that for all $ \zeta $ with $ s \leq \abs{ \zeta } < 1 $,
\begin{equation}
 \abs{ \ph' (\zeta) } \leq C_s \p{ 1 - \abs{ \zeta } }^{ - 1 }.
\end{equation}


Recall that for all $ n \geq 0 $ and all $ \zeta \in V $,
 $ P^n \composedwith \ph (\zeta) = \ph \p{ \zeta^{d^n} } $.
 In particular it follows that if $ \xi = \zeta^{ d^n } $,
 \begin{equation}
  \p{ P^n }' (\ph (\zeta)) \ph' (\zeta) = d^n \frac{ \xi }{ \zeta } \ph' (\xi).
 \end{equation}

Fix $ 0 < r < 1 $ and suppose that $ r^2 \leq \abs{ \xi } \leq r $.
Then
\begin{equation}
 \abs{ \p{ P^n }' (z) } \geq d^n r^2 C_{ r^2 }^{ -1 } \p{ 1 - \abs{ \zeta } } \abs{ \ph' (\xi) }
\end{equation}
with $ z = \ph (\zeta) $.
Since $ r $ is fixed, $ \abs{ \ph' (\xi) } $ is bounded away from $ 0 $ and $ \infty $ by a constant independent of $ \xi, \zeta $ and $ n $.
For the same reason, $ 1 - \abs{ \zeta } $ is comparable to $ d^{ -n } $ with constants independent from $ \xi, \zeta $ and $ n $.
Hence $ \abs{ \p{ P^n }' (z) } $ is bounded away from $ 0 $ by a constant independent from $ \xi, \zeta $ and $ n $.
Now one can apply this with $ w = \ph (\xi) $.
\end{proof}

















































HERE...

\begin{cor} \label{cor:ehypdim is strictly smaller for L}
Let $ P : \complexnumbers \rightarrow \complexnumbers $
 be a polynomial of degree at least $ 2 $ which is topologically Collet-Eckmann
 and whose Julia set is connected.
Let $\poincarefunction$
 be a Poincar{\'e} function associated to a repelling fixed point of $ P $.
Then,
\begin{equation*}
 \evhypdim \poincarefunction < \hypdim \poincarefunction.
\end{equation*}
\end{cor}


\wip{TODO: check this whole proof a last time}
\begin{proof}
 Let's first introduce many notations.
 Fix $r_0>0$ small so that the restriction of $ \poincarefunction $
 to the disk $ \Disk (0, |\multiplier|^2 r_0)$ is univalent.
 Let for all $ i \in \integers_{ \geq 0 } $,
 \begin{equation}
  A_i \defeq \setof{ z \in \complexnumbers : \abs{ \multiplier }^i r_0 \leq \abs{ z } < \abs{ \multiplier }^{ i + 1 } r_0 }
 \end{equation}
and
\begin{equation}
 A_P \defeq L (A_0).
\end{equation}

Let $ \basin (\infty) $ be the basin of $ \infty $  of $ P $.
Since the Julia set of $ P $ is connected
 there exists a conformal isomorphism
 $ \psi $
 from the basin of $ \infty $ of $ P $ onto the complement of the closed unit disk which conjugates $ f $ to $ z \mapsto z^d $.
 Since $ 0 $ is a repelling fixed point of $ P $  there exists an external ray $ \gamma $
 landing at $ 0 $,
 say of angle $ \theta_0 $.
 Let $ 1 < r_- < r_+  $ be such that
 $ \gamma \intersection A_P = \psi^{ -1 } \p{ \setof{ r e^{ i \theta_0 } : r_- \leq r < r_+ } } $.
 
Let $ \theta_- < \theta_0 < \theta_+ $ be such that
 the intersections of 
 $ \psi^{ -1 } \p{ \setof{ r e^{ i \theta } : r >  1, \theta_- < \theta < \theta_+ } }  $
 with the inner and outer boundary of the annulus $ A_P $
 both contain a set of the form
 $ \psi^{ -1 } \p{ \setof{ r (\theta) e^{ i \theta } : \theta_- < \theta < \theta_+ } } $
 with $ r (\theta) $ being  some function dependant on which boundary we consider.
 

Let 
$ \theta_- < \theta_{-0} < \theta_{-+} < \theta < \theta_{++} < \theta_{+0} < \theta_+ $.
Define the following sets:
 \begin{align}
  U_- & \defeq A_P \intersection \psi^{ -1 } \p{ \setof{ r e^{ i \theta } : r >  1, \theta_- < \theta < \theta_+ } }  \\
  U_0 & \defeq A_P \intersection \psi^{ -1 } \p{ \setof{ r e^{ i \theta } : r >  1, \theta_{-0} < \theta < \theta_{+0} } }  \\
  U_+ & \defeq A_P \intersection \psi^{ -1 } \p{ \setof{ r e^{ i \theta } : r >  1, \theta_{-+} < \theta < \theta_{++} } }.
 \end{align}
Then by construction $ U_-, U_0 $ and $ U_+ $ are connected simply connected subsets of $ A_P \intersection \basin (\infty) $
connecting both boundaries of $ A_P $.
 


Define for $ i \in \integers_{ \geq 0 } $
\begin{align}
 B^+_i   &   \defeq   \setof{ z = \rho^i \zeta :
                                 \zeta \in A_0,
                                 r_0 < \abs{ \zeta }
                                 \mbox{ and } L (\zeta) \notin U_+ }, \\
  B_i    &   \defeq   \setof{ z = \rho^i \zeta :
                                 \zeta \in A_0,
                                 (1 + \eps) r_0 < \abs{ \zeta } < (1 - \eps) r_0 \abs{ \multiplier }
                                 \mbox{ and }
                                 L (\zeta) \notin U_0 }, \\
  B^-_i  &   \defeq  \setof{ z = \rho^i \zeta :
                                 \zeta \in A_0,
                                 (1 + 2 \eps) r_0 < \abs{ \zeta } < (1 - 2 \eps) r_0 \abs{ \multiplier }
                                 \mbox{ and }
                                 L (\zeta) \notin U_- }.
\end{align}
We assume that $ \eps > 0 $ is small enough so that $ B^-_0 \neq \emptyset $.
Note that by construction $ B^-_i $, $ B^+_i $ and $ B_i $ are simply connected open subsets of $ \complexnumbers $.
We assume that $ B_i $ is connected (otherwise take the biggest connected component).

Now let $ n \in \integers_{ \geq 1 } $ be large enough so that
for all $ i \geq n $, $ B_i $ does not intersects the singular set of $ L $.
We consider the family $ \mathcal{Q} = \mathcal{Q} (n) $ of simply connected open sets $ Q \subset \complexnumbers $
 such that there exists $ i $ and $ j $ in $ \setof{ n, n + 1, \dots, 2 n } $
 such that 
 $ Q \subset B_j $,
 $ Q \intersection B^-_j \neq \emptyset $
 and the mapping $ L : Q \to B_i $ is a conformal isomorphism.
 For each $ Q \in  \mathcal{Q} $ we define
 \begin{equation}
  \ph_Q \defeq L_{ \restricted Q }^{ - 1 }.
 \end{equation}

 
 We will show that if $ n $ is large enough,
 the system of mappings $ \family{ \ph_Q }_{ Q \in \mathcal{Q} } $
 generates a conformal graph directed Markov system (CGDMS) and that
 the dimension of the limit set of this CGDMS is greater than
 \begin{equation}
  h \defeq \hypdim \poincarefunction.  
 \end{equation}
 For background on CGDMS compare \cite{MauldinUrbanski2003}. % should be the book ``Graph Directed Markov Systems''
 Moreover the limit set of the GCDMS will be an hyperbolic set for $ L $.



 Firstly assume that $ Q $ is an open connected set such that
 there exists $ Q_+ $ and
 some $ i, j \geq n $,
 such that
 $ L : Q_+ \to B_i^+ $  is a conformal isomorphism,
 $ Q \subset Q_+ $,
 $ L (Q) = B_i $
 and $ Q \intersection B_j \neq \emptyset $.
 We will show that by choosing $ n $ large enough,
 the mapping $ L $ is expanding
  with constants independent of $ Q, i, j $.
  Define as above $ \ph_{ Q } \defeq \p{ L_{ \restricted Q } }^{ -1 } $.
Note that there is a uniform bound on the distortions of the maps $ \ph_Q $, 
 measured in terms of the cylinder metric,
 independent of $ Q, i, j $.


  
 

Our first step is to estimate the norm of the derivative of the maps $ \ph_Q $ with respect to the cylinder metric.
We fix $ R > 1 $ and let $ F $ be the image of a ring $ \setof{ R < \abs{ z } \leq R^2 } $
 by the inverse of the B{\"o}ttcher coordinates at $ \infty $ for $ P $.
 Then there exists $ C_{\mbox{mono}} > 1 $ such that 
 for all $ \xi $ in the unbounded component of the complement of $ F $ and for all $ k \in \integers_{ \geq 0 } $
 \begin{equation} \label{eq: the derivative of the polynomial is comparable to the derivative of the high order monomial}
  C_{\mbox{mono}}^{ - 1 }
  \leq 
  \abs{ \frac{ \p{ P^k }' (\xi) }{ d^k P^k (\xi) / \xi } }
  \leq
  C_{\mbox{mono}}.
 \end{equation}
Note that by construction if $ w $ and $ \nu $ are such that $ P^{ - \nu } (w) \intersection F \neq \emptyset $
then $ P^{ - \nu } (w) \subset F $.
For all $ w $ in the unbounded component of the complement of $ F $,
let $ \nu_F = \nu_F (w) $ be the unique positive integer such that $ P^{ - \nu_F } (w) \subset F $.
Then there exists $ C_{ F } \in \realnumbers $
 independent of $ w $
 such that
\begin{equation}
 \frac{ \log \log \abs{ w } - C_{ F } }{ \log d } \leq \nu_F \leq \frac{ \log \log \abs{ w } + C_{ F } }{ \log d }.
\end{equation}
 We also assume $ n $ is large so that $ F $ is in the bounded component of the $ A_n $.
 
 Let $ i, j \in \setof{ n, \dots, 2 n } $ and let
 $ z \in B_j $ be such that $ L (z) \in B_i $.
 Then from Observation \ref{obs:preimage structure}
 it follows that
 $ L' (z) = \frac{ 1 }{ \rho^j } \p{ P^j }' (\zeta) L' (z / \rho^j) $
 where $ \zeta \in A_P $ is 
 \wip{ $ \zeta = L \p{ z / \rho^j } $. }
 Let $ w = L (z) $, $ \nu = \nu_F (w) $ and $ \xi = P^{ j - \nu } (\zeta) $.
 Then
 \begin{equation}
  \cylnorm{ \Deriv L (z) } = \abs{ L' (z / \rho^j) \frac{ z }{ \rho^j } \frac{ \p{ P^{ \nu } }' (\xi) }{ w } \p{ P^{ j - \nu } }' (\zeta) }. 
 \end{equation}
The factor $ \abs{ L' (z / \rho^j) \frac{ z }{ \rho^j } } $ is comparable to a constant independently from $ i, j, z, n $.
By \eqref{eq: the derivative of the polynomial is comparable to the derivative of the high order monomial}
 the term $ \abs{ \frac{ \p{ P^{ \nu } }' (\xi) }{ w } } $
 is comparable to $ d^{ \nu } \approx \log \abs{ w } $ independently from $ i, j, z, n $.
 Hence there exists $ C_{ deriv } > 1 $ independent from $ i, j, n, z, \zeta $ such that
 \begin{equation}
  C_{ deriv }^{ -1 } %\log \abs{ w } \abs{ \p{ P^{ j - \nu } }' (\zeta) }
  \leq
  \frac{ \cylnorm{ \Deriv L (z) } }{ \abs{ \p{ P^{ j - \nu } }' (\zeta) }  \log \abs{ w } }
  \leq
  C_{ deriv } .
 \end{equation}
  Moreover it follows from Lemma \ref{lem: derivative of polynomial bounded from below on the basin of infinity}
  that $ \abs{ \p{ P^{ j - \nu } (\zeta) }' } $ is bounded from below away from $ 0 $
  independently from $ i, j, \zeta, z, n $.
 
 
 Hence if $ n $ is large enough there exists $ k_{ \mathcal{Q} } > 1 $
 such that for all $ Q \in \mathcal{ Q } $ and all $ z $ in the domain of $ \ph_Q $,
 $ \cylnorm{ \Deriv \ph_Q (z) } \leq k_{ \mathcal{Q} }^{ - 1 } $.
 Moreover $ k_{ \mathcal{Q} } \tendsto \infty $ as $ n \tendsto \infty $.
 

Remark that the diameter of $ B_i $ is uniformly bounded independently from $ i $ with respect to the cylindrical metric.
 It follows that for any $ \eta > 0 $ one can find $ n $ such that
 the cylindrical diameter of $ \ph_Q (B_i) $ is smaller than $ \eta $.
 
We use this to show that the system is not empty for $ n $ large enough.
 Choose for any $ i \geq $ a point $ c_i \in B_{i}^- $.
 Then from Observation \ref{obs:preimage structure} and Proposition \ref{prop:???}
 it follows that $ L^{ -1 } (c_i) \intersection B_j $ 
 is not empty for any $ j \geq n $
 and $ n $ large enough (independently of $ i $).
 
By the previous considerations this means that on can find $ Q $ as above such that
$ \ph_Q (B_i) \subset B_j $. 
This shows that not only the system is not empty but also that it is $ 2 $-irreducible.
Hence we have an irreducible CGDMS.
We can estimate the dimension of its limit set by using thermodynamical formalism.

Indeed 
let's compute the $p$th partition function with respect to the cylinder metric:
\begin{align*}
 & 
  \familysum{i_1=n}{\widthconst n}
  \cdots
  \familysum{i_{p+1}=n}{\widthconst n}
  \familysum{\alpha_1=1}{\alpha_{i_1,i_2}}
   \cdots
  \familysum{\alpha_p=1}{\alpha_{i_p,i_{p+1}}}
   \left\| \left(\ph_{i_1,i_2,\alpha_1}
                 \composedwith \cdots \composedwith
                 \ph_{i_p,i_{p+1},\alpha_p}\right)' \right\|_{\cyl}^t \\
  & \geq
  \kappa_1
  \familysum{i_1=n}{\widthconst n}
  \cdots
  \familysum{i_{p+1}=n}{\widthconst n}
  \familysum{\zeta_1\in A_0\intersection P^{-i_1}(A_{i_2})}{}
  \cdots
  \familysum{\zeta_p\in A_0\intersection P^{-i_p}(A_{i_p+1})}{}
   (i_1\cdot\dots\cdot i_p)^{-t}
   \left|P^{i_1-\nu_{i_2}}(\zeta_1)\right|^{-t}
   \cdot \dots \cdot
   \left|P^{i_p-\nu_{i_{p+1}}}(\zeta_p)\right|^{-t} \\
  & \geq
  \kappa_2
  \familysum{i_1=n}{\widthconst n}
  \cdots
  \familysum{i_{p+1}=n}{\widthconst n}
   n^{-p t}
   \partitionfunction(P^{i_1-\nu_{i_2}}_{\restricted N},t)
   \cdot \dots \cdot
   \partitionfunction(P^{i_p-\nu_{i_{p+1}}}_{\restricted N},t) \\
  & \geq
   \kappa_3 n^{p(1-t)+1}.
\end{align*}
(where $\kappa_i>0$ are constants independent of $n,p$).

 

 



\end{proof}































==> math-lib.tex <==



\usepackage{bbm}

\usepackage{calrsfs}

\usepackage{color}


\usepackage{hyperref}

\usepackage{enumitem}
\setenumerate[1]{label={\arabic*.}}




\numberwithin{equation}{section}

\newcommand{\hide}[1]{}

\newcommand{\comment}[1]{{\leavevmode\color{green}{#1}}}


\newcommand{\eps}{\varepsilon}
\renewcommand{\epsilon}{\eps}
\newcommand{\ph}{\varphi}
\renewcommand{\phi}{\ph}

\newcommand{\khi}{\chi}
\newcommand{\thetau}{{2 \pi}}

\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt
                     \hbox{\scriptsize.}\hbox{\scriptsize.}}}%
                     =}
\newcommand{\eqdef}{=\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt
                     \hbox{\scriptsize.}\hbox{\scriptsize.}}}}



\newcommand{\ontop}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}

\newtheorem{thm}{Theorem}[section]

\newtheorem{claim}[thm]{Claim}
\newtheorem{claims}[thm]{Claims}
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem{conjectures}[thm]{Conjectures}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{corollaries}[thm]{Corollaries}
\newtheorem{definition}[thm]{Definition}
\newtheorem{definitions}[thm]{Definitions}
\newtheorem{defn}[thm]{Definition}
\newtheorem{defns}[thm]{Definitions}
\newtheorem{example}[thm]{Example}
\newtheorem{examples}[thm]{Examples}
\newtheorem{exple}[thm]{Example}
\newtheorem{exples}[thm]{Examples}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{lemmas}[thm]{Lemma}
\newtheorem{obs}[thm]{Observation}
\newtheorem{observation}[thm]{Observation}
\newtheorem{observations}[thm]{Observations}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{props}[thm]{Propositions}
\newtheorem{question}[thm]{Question}
\newtheorem{questions}[thm]{Questions}
\newtheorem{rem}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{remarks}[thm]{Remarks}
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{theorems}[thm]{Theorems}

\newcommand{\termdefined}[1]{\textbf{#1}}




\newcommand{\equivalent}{\Leftrightarrow}
\newcommand{\ifandonlyif}{\equivalent}

\newcommand{\freevariable}{\placeholder}


\newcommand{\setof}[1]{\left\{#1\right\}}

\newcommand{\contains}{\supset}

\newcommand{\setcomplement}{{\mathbin{\backslash}}}
\newcommand{\setintersection}{\mathbin{\cap}}
\newcommand{\setunion}{\mathbin{\cup}}


\newcommand{\composedwith}{\mathbin{\circ}}
\newcommand{\graph}{\operatorname{Graph}}
\newcommand{\identitymap}{\operatorname{id}}
\newcommand{\indicatorfunction}{{\mathbbm{1}}}
\newcommand{\mapdomain}{\operatorname{dom}}
\newcommand{\restricted}{|}

\newcommand{\cardinalnumber}{\operatorname{Card}}
\newcommand{\numberofelements}{\#}

\newcommand{\family}[2]{\left(#1\right)_{#2}}
\newcommand{\familydisjointunion}[2]{{\bigsqcup\limits_{#1}^{#2}}\ }
\newcommand{\familyintersection}[2]{{\bigcap\limits_{#1}^{#2}}\ }
\newcommand{\familyunion}[2]{{\bigcup\limits_{#1}^{#2}}\ }


\newcommand{\complexnumbers}{{\mathbbm{C}}}
\newcommand{\integers}{{\mathbbm{Z}}}
\newcommand{\naturalnumbers}{{\mathbbm{N}}}
\newcommand{\rationalnumbers}{{\mathbbm{Q}}}
\newcommand{\realnumbers}{{\mathbbm{R}}}



\newcommand{\nonzerocomplexnumbers}{{{{\complexnumbers_{\neq 0}}}}}
\newcommand{\nonzeronaturalnumbers}{{{{\naturalnumbers_{\neq 0}}}}}
\newcommand{\nonzerorealnumbers}{{{{\realnumbers_{\neq 0}}}}}

\newcommand{\negativerealnumbers}{{\realnumbers_{<0}}}
\newcommand{\nonnegativeintegers}{{\integers_{\geq 0}}}
\newcommand{\nonnegativerealnumbers}{{\realnumbers_{\geq 0}}}
\newcommand{\positiveintegers}{{\integers_{>0}}}
\newcommand{\positiverealnumbers}{{{{\realnumbers_{>0}}}}} % LATEX

\newcommand{\positivezintegers}{{\integers_{\geq 0}}}
\newcommand{\positivezrealnumbers}{{\realnumbers_{\geq 0}}}
\newcommand{\negativesrealnumbers}{{\realnumbers_{<0}}}
\newcommand{\positivesintegers}{{\integers_{>0}}}
\newcommand{\positivesrealnumbers}{{{{\realnumbers_{>0}}}}} % LATEX

\newcommand{\integerinterval}[2]{{\setof{{#1},\dots,{#2}}}}
\newcommand{\integersmodulo}[1]{\integers_{#1}}

\newcommand{\absolutevalue}[1]{\left|#1\right|}
\newcommand{\ceilingfunction}[1]{\left\lceil#1\right\rceil}
\newcommand{\integerpart}[1]{\left\lfloor#1\right\rfloor}


\newcommand{\argumentplaceholder}{\cdot}
\newcommand{\coarser}{\succ}
\newcommand{\completion}[1]{\overline{#1}}
\newcommand{\dimension}{\operatorname{dim}}
\newcommand{\finer}{\prec}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\placeholder}{\cdot}
\newcommand{\prioritize}[1]{\left(#1\right)}
\newcommand{\wavyequality}{\approx}



\newcommand{\sequence}[1]{\left(#1\right)}
\newcommand{\tendsto}{{\to}}
\newcommand{\topologicalboundary}{{\partial}}
\newcommand{\topologicalclosure}[1]{\completion{#1}}
\newcommand{\topologicalinterior}[1]{\operatorname{Int} \p{#1}}

\newcommand{\closedinterval}[1]{\left[#1\right]}
\newcommand{\closedopeninterval}[1]{\left[#1\right[}
\newcommand{\openclosedinterval}[1]{\left]#1\right]}
\newcommand{\openinterval}[1]{\left]#1\right[}


\newcommand{\familyinf}[1]{{\inf\limits_{#1}}\ }
\newcommand{\familyproduct}[2]{{\prod\limits_{#1}^{#2}}\ }
\newcommand{\familysum}[2]{{\sum\limits_{#1}^{#2}}\ }
\newcommand{\familysup}[1]{{\sup\limits_{#1}}\ }

\newcommand{\ball}{B}
\providecommand{\diameter}{\operatorname{diam}}
\newcommand{\disk}{D}
\newcommand{\distance}{\operatorname{dist}}
\newcommand{\norminfty}[1]{\norm{#1}_\infty}



\newcommand{\absolutelycontinuouswrt}{{\ll}}
\newcommand{\dirac}{\delta}
\newcommand{\lebesguemeasure}{\operatorname{Leb}}
\newcommand{\oldintegral}[4]{\int_{#1}^{#2} #3 \,{\rm \differential} #4}
\newcommand{\integraloperator}[3]{\int_{#1}^{#2} \,{\rm \differential} #3\,}
\newcommand{\volume}{\operatorname{Vol}}


\newcommand{\comparable}{\wavyequality}
\newcommand{\derivative}{{\rm D}}
\newcommand{\differentiabilityclass}{\smoothclass}
\newcommand{\differential}{{\rm d}}
\newcommand{\bigo}{O}
\newcommand{\fourier}[1]{\widehat{#1}}
\newcommand{\littleo}{o}
\newcommand{\partialderivative}[2]{{\frac{\partial #1}{\partial #2}}}
\newcommand{\smallo}{\littleo}
\newcommand{\smoothclass}{C}
\newcommand{\support}{\operatorname{supp}}





\newcommand{\expectedvalue}{{\mathbb{E}}}




\newcommand{\normLp}[2]{\norm{#1}_{#2}}
\newcommand{\normLinfinity}[1]{\normLp{#1}{\infty}}
\newcommand{\sobolevspace}[2]{W^{#1,#2}}
\newcommand{\sobolevspaceloc}[2]{\sobolevspace{#1}{#2}_{loc}}



\newcommand{\laplace}{\Delta}



\newcommand{\area}{\operatorname{area}}
\newcommand{\length}{\operatorname{length}}
\newcommand{\projectivespace}{\mathbb{P}}
\newcommand{\sphere}{{\mathbb{S}}}
\newcommand{\torus}{{\mathbb{T}}}



\newcommand{\boxdimension}{\operatorname{BD}}
\newcommand{\fourierdimension}{\dimension_F}
\newcommand{\hausdorffcontent}{{\hausdorffmeasure_c}}
\newcommand{\hausdorffdimension}{\operatorname{HD}}
\newcommand{\hausdorffmeasure}{\mathcal{H}}
\newcommand{\lowerboxdimension}{{\underline{\operatorname{BD}}}}
\newcommand{\packingdimension}{\operatorname{PD}}
\newcommand{\packingmeasure}{\Pi}
\newcommand{\packingonlydimension}{\operatorname{P^*D}}
\newcommand{\upperboxdimension}{{\overline{\operatorname{BD}}}}



\newcommand{\annulus}{A}
\newcommand{\complexconjugate}[1]{\overline{#1}}
\newcommand{\complexplane}{\complexnumbers}
\newcommand{\dcomplex}{\partial}
\newcommand{\dcomplexbar}{\complexconjugate{\partial}}
\newcommand{\imaginarypart}{\operatorname{Im}}
\newcommand{\maximummodulus}{M}
\newcommand{\mobiustransforms}{\operatorname{Mob}a}
\newcommand{\realpart}{\operatorname{Re}}
\newcommand{\riemannsphere}{\widehat{{\complexnumbers}}}
\newcommand{\squarerootofminusone}{i}
\newcommand{\sqrtmone}{{\squarerootofminusone}}
\newcommand{\twopii}{2\pi\sqrtmone}
\newcommand{\unitdisk}{{\mathbb{D}}}
\newcommand{\upperhalfplane}{\mathbb{H}}


\newcommand{\beltramiform}[1]{\frac{\dcomplexbar{#1}}{\dcomplex{#1}}}
\newcommand{\logarithmicmeasure}{\operatorname{lm}}



\newcommand{\bryunonumbers}{\mathcal{B}}
\newcommand{\iterated}{}
\newcommand{\rotationnumber}{\rho}



\newcommand{\partitionfunction}{Z}
\newcommand{\pressure}{P}





\newcommand{\bryunofunction}{\mathcal{B}}
\newcommand{\classb}{\mathcal{B}}
\newcommand{\escapingset}{I}
\newcommand{\fatouset}{F}
\newcommand{\filledjuliaset}{K}
\newcommand{\hermannumbers}{\mathcal{H}}
\newcommand{\hyperbolicdimension}{\operatorname{hypdim}}
\newcommand{\juliaset}{J}
\newcommand{\mandelbrotset}{M}
\newcommand{\postsingularset}{{\operatorname{PSS}}}
\newcommand{\radialjuliaset}{{\juliaset}_{\operatorname{r}}}
\newcommand{\speiserclass}{\mathcal{S}}






\newcommand{\continuedfraction}[1]{\left[#1\right]}
\providecommand{\divides}{|}
\providecommand{\notdivides}{{\not \divide}}



\newcommand{\plusorminus}{\pm}

\newcommand{\abs}[1]{\absolutevalue{#1}}
\newcommand{\absolutelycontinuous}{\absolutelycontinuouswrt}
\newcommand{\boundary}{\topologicalboundary}
\newcommand{\card}{\numberofelements}
\newcommand{\closure}{\topologicalclosure}
\newcommand{\diam}{\diameter}
\newcommand{\interior}{\topologicalinterior}
\newcommand{\intersection}{\setintersection}
\newcommand{\hypdim}{\hyperbolicdimension}
\newcommand{\jrad}{\radialjuliaset}
\newcommand{\mandelbrot}{\mandelbrotset}
\newcommand{\noarg}{\argumentplaceholder}
\newcommand{\p}{\prioritize}
\newcommand{\postsingular}{\postsingularset}
\newcommand{\set}{\setof}
\newcommand{\union}{\setunion}


\newcommand{\cyl}{\operatorname{cyl}}
\newcommand{\eucl}{\operatorname{eucl}}
\newcommand{\hyp}{\operatorname{hyp}}
\newcommand{\sph}{\operatorname{sph}}

\newcommand{\modd}[1]{|{\rm d}#1|}








